Architectural Decay as Predictor of Issue- and Change-Proneness

Architectural decay imposes real costs in terms of developer effort, system correctness, and performance. Over time, those problems are likely to be revealed as explicit implementation issues (defects, feature changes, etc.). Recent empirical studies have demonstrated that there is a significant correlation between architectural "smells" -- manifestations of architectural decay -- and implementation issues. In this paper, we take a step further in exploring this phenomenon. We analyze the available development data from 10 open-source software systems and show that information regarding current architectural decay in these systems can be used to build models that accurately predict future issue-proneness and change-proneness of the systems' implementations. As a less intuitive result, we also show that, in cases where historical data for a system is unavailable, such data from other, unrelated systems can provide reasonably accurate issue- and change-proneness prediction capabilities.

==> 4.3.predict.tex <==
\chapter{Speculative Analysis to Predict Impact of Architectural Decay on the Implementation of Software Systems}
\label{sec:prediction}

\section{Foundation}
\label{sec:emp3_found}
This chapter discusses the dissertation's third large study, which aims to solve a prediction problem by using 
%The prediction problem, which this chapter will address, is under the umbrella of 
supervised machine learning (ML) techniques. In supervised learning, ML systems learn how to combine input to produce useful predictions of data which has not been seen before. 
In particular, we would like to predict the impact of architectural decay on the implementation of software systems. 
In this prediction problem, the input features are architectural smells of a system and the output features, i.e., labels, are the issue- and change-proneness of that system. This section will describe two steps to pre-process the raw data before it is used in supervised ML algorithms. The two pre-processing steps are (1) labeling implementation's properties and (2) balancing the datasets. 
%In addition, this section \rhl{or chapter} will also introduces the evaluation metrics used in this study to asses the accuracy of the prediction models. 


\subsection{Labeling Data}
\label{sec:labeling}
Labeling data is a crucial step to ensure the success of building prediction models. 
In our prediction problem, the raw information of a system's implementation includes the numbers of issues and changes of each source file. Nonetheless, these numbers could not be used directly as predicted labels  because intuitively it would be impossible to build a model which can accurately predict a precise number of issues or changes. Rather than that, those numbers have to be converted %of issues and changes 
to nominal labels which represent the levels of issue- and change-proneness. 

The way to convert a set of numeric values to nominal labels depends on the distribution of the numeric values. In our problem, the numbers of issues and changes of a system follow a heavy-tailed distribution \cite{heavy-tailed}. These distributions are often segmented into ranges. Most simply and commonly, a distribution can be divided into two segments, which are the head and the tail. A more sophisticated approach is to divide the distribution into three parts, which are the head, the body, and the tail. This study uses the three-segment division, which represents three levels of proneness: low, medium, and high. This approach is chosen because of its potential to give developers a better estimation of architectural decay's impact. To segment a dataset, this study uses the Pareto principle \cite{pareto}, a popular segmentation method for heavy-tailed distributions. This principle is also widely used in software engineering, particularly value-based software engineering \cite{boehm2006value}. To obtain three segments, the Pareto principle is repeatedly applied two times %to itself 
as suggested in the literature \cite{arthur2001six}. 

%\rhl{
To collect the data regarding architectural decay, this study uses the approach already applied in the second study of this dissertation on architectural decay.
More specifically
%To obtain the raw data%for answering this study's research questions
, for each version of a subject system, we first collect the list of issues which affects that version. Similar to the second study%on architectural decay
, only ``resolved'' and ``fixed'' issues are taken into account. Then the files that were changed in order to fix the issues are collected. For each file, we gather its associated architectural smells (determined by the triad relationships of issues, files, and smells in Figure \ref{fig:issue_smell_mapping}), the number of issues whose fixing commits changed the file, and the total number of changes.%}
After the raw data is collected, it has to be labeled 
%and balanced 
using the Pareto technique mentioned above %in Section \ref{sec:emp3_found} %.preprocessed 
before being fed to supervised ML algorithms. 
%The raw data then be 
Specifically, to determine the level of issue-proneness of a source file in a software version, first, the number of issues related to that source file %in that version 
is collected. This is considered as one data point. We collect data points for all files in all versions of a software system, and then sort the dataset by the numbers of issues, from low to high.
%a dataset is sorted by the number of issues (or changes) from low to high. 
Then, the first 80\% of data points are marked with ``low'' labels. Finally, the next 16\% (80\% of 20\%) and 4\% (20\% of 20\%) of data points are marked with ``medium'' and  ``high'' labels respectively. Similarly, to determine the change-proneness of a source file in a software version, we count the number of commits related to that file and repeat the labeling process like above.
%(or changes)
%(or change-proneness) 


Table \ref{tab:data_point_sample} shows a few data samples in our datasets after labeling. All the eleven architectural smells in the second empirical study of this dissertation are considered as the input features of this third study. 
The examples of input features in Table \ref{tab:data_point_sample} are CO (Concern Overload), SPF (Scattered Parasitic Functionality), LO (Link Overload), and DC (Dependency Cycle) smells. The output features, i.e., labels, are the levels of issue- and change-proneness.  %Two output features are issue-proneness and change-proneness.
%\rhl{
The two leftmost columns show the versions and the filenames of data points. The next eleven columns are binary features which indicate whether or not the files have a specific smell. ``1'' means having the smell, and ``0'' is the other way around. 
%Later, the issues proneness indicate numbers of issues which appear in that version, then later have to fix by changing the files. 
The two rightmost columns indicate the issue- and change-proneness of the files. For example, in version 0.20.0 of Hadoop, DFSClient.java has three smells: Scattered Parasitic Functionality, Link Overload, and Dependency Cycle. The file's issue-proneness is high, and its change-proneness is low.%}


\begin{table*}[th]
	\centering
	\caption{Data Samples of Hadoop}
	\label{tab:data_point_sample}
	\begin{tabular}{|l|l|l|l|l|l|l|p{1.5cm}|p{1.5cm}|}
		\hline
		Version &  Filename        & CO & SPF & LO & DC & ... & Issue-proneness & Change-proneness \\ \hline
		0.20.0 & hadoop/dfs/DFSClient.java & 0                & 1   & 1             & 1                & ... & high            & low              \\ \hline
		0.20.0 & hadoop/mapred/JobTracker.java         & 1                & 0   & 1             & 0                & ... & medium             & medium              \\ \hline
		0.20.0 & hadoop/tools/Logalyzer.java       & 0                & 0   & 0             & 0                & ... & low             & low              \\
		\hline      
		... & ...       & ...                & ...   & ...             & ...                & ... & ...             & ...              \\
		\hline      
	\end{tabular}
\end{table*}

\subsection{Balancing Data}
Because of the data's distribution and the labeling approach, the datasets in this third study are mostly unbalanced. %\rhl{
Recall from Section \ref{sec:labeling} that %because of the Pareto principle, 
the ``low'':``medium'':``high'' ratio of our datasets is 80:16:4 (i.e., 20:4:1). If a dataset with that ratio is used to train a prediction model, the model will tend to predict ``low'' every time, with an 80\% chance of being correct. %} 
For this reason, it is very important to balance these datasets to ensure that weighted metrics are not biased by less (or more) frequent labels. This dissertation use SMOTE \cite{chawla2002smote} to balance our datasets. 
Details of SMOTE has been described in Section \ref{sec:ml_found}.
For our specific problem, % To solve this problem, 
SMOTE is used to oversample ``medium'' by a factor of 5 and ``high'' by a factor of 20. After oversampling, the dataset will be balanced and its ``low'':``medium'':``high'' ratio will be 1:1:1.


\section{Research Question and Hypotheses}
The two empirical studies of software architectural changes and decay in this dissertation (Section \ref{sec:empirical_change} and Section \ref{sec:empirical_decay}) have answered some key research questions in software architecture community and confirmed the visible impact of architectural decay on software systems' implementation. The decay's impact %on implementation, which 
reveals itself in the form of correlations with %implementation issues%with 
systems' issue-proneness and change-proneness. This is the cornerstone for exploring further research questions.
%about correlations between impact of architectural smells and issues.
Specifically, that finding has provided the intuition for the third study in this dissertation, which attempts to create an architectural-based approach to predicting the decay's impact on a system's implementation. %Consequently, 
The following hypothesis about the approach has been developed.

\textbf{Hypothesis}: {It is possible to construct accurate models to predict the impact of architectural smells on systems' implementation. }

To prove this hypothesis, this study particularly focuses on %building prediction models to 
the predictability of the issue-proneness and change-proneness of a system based on its architectural smells. This decision is based on the result of this dissertation's second empirical study, which showed the significant correlations between architectural smells and those two properties. The two following research questions have been defined accordingly.


\textit{\textbf{RQ1.}} To what extent can the architectural smells detected in a system help to predict the issue-proneness and change-proneness of that system at a given point in time?

%\rhl{
The training data used to build the prediction models of a system is collected from different versions of that system during its lifetime. Therefore, if these models can yield high accuracy in predicting issue- and change-proneness, this indicates that architectural smells have consistent impacts on those two properties throughout the system's lifecycle. 
This is very important because it ensures that the impact of architectural smells is not related to other factors, such as the system's size, which may change during the system's evolution. In addition, a highly accurate prediction model will be useful for developers to foresee the future issue-proneness and change-proneness of newly smell-affected parts of the system. The prediction models will also be useful for the system's maintainers in order to decide when and where to refactor the system. For example, the maintainers can use the models to estimate the reduction of the issue- and change-proneness if they remove some smell instances from the system's implementation. 
%}

\textit{\textbf{RQ2.}} To what extent do unrelated software systems tend to share properties with respect to issue- and change-proneness?

This research question aims to determine whether architectural smells have similar impacts on the implementations of different systems. Specifically, we would like to see if the issue- and change-proneness of a system can be accurately predicted by a ``general-purpose'' model trained by the datasets of other software systems. If this hypothesis is confirmed, 
architectural smell-based models can be reused 
by developers to predict the issue- and change-proneness of new software systems in the early stages of their development, before sufficiently large numbers of system versions become available. 
%will be universal indicators of issue- and change-proneness in software systems.  
%\rhl{
Moreover, we would like to see how different combinations of systems result in the accuracy of the general-purpose models.%} 

To answer these two research questions, we need to %\rhl{
build different prediction models based on the data regarding architectural smells %} 
and then determine how accurate these models are. First, we collect the data regarding architectural decay of the subject systems as well as their issue- and change-proneness. Then we apply different machine learning techniques %\rhl{
and use accuracy metrics to %} 
evaluate their effectiveness in building prediction models in the context of this study. The models' accuracy will be measured under different architectural views to see how different architectural recovery techniques affect the prediction models. %\rhl{
Similar to the first two empirical studies in this dissertation, this study uses three architectural recovery methods: ACDC \cite{tzerpos2000}, ARC \cite{garcia2011enhancing}, and PKG \cite{leempirical}.%}

%\rhl{
%\subsection{Evaluation Metrics}
To evaluate the accuracy of prediction models, we use three widely accepted metrics: precision, recall, and f-score \cite{powers2011evaluation}. Precision is the fraction of correctly predicted labels over all predicted labels. Recall is the fraction of correctly predicted labels overall actual labels. Finally, f-score is the harmonic mean of precision and recall to represent a test's accuracy. 

We use two different approaches to obtain evaluation results. The first approach uses two independent datasets: a training set and a test set. The second approach uses only a dataset with cross-validation setup. For the second approach, this study uses 10-fold-cross-validation, where the dataset is randomly divided into ten equal-sized subsets. Then we sequentially select one subset and test it against the prediction model built by the other nine subsets. The final result is the mean of ten tests' results. 
%}

To facilitate the whole process, this study uses ARCADE (Section \ref{sec:arcade})---our framework to study software architecture---to collect raw data, and WEKA\cite{weka}---a well-known ML framework---to pre-process data, build prediction models and evaluate the models' accuracy.

\section{Subject Systems} 

In order to answer the above research questions, we use the data collected from the subject systems in the second empirical study (Section \ref{sec:empirical_decay}) of this dissertation. Table %\ref{tab:subject_systems_predict}
\ref{tab:subject_systems} shows the list of seven subject systems. % from the empirical study of architectural decay , which will be reused to build prediction models. 
One system, Continuum, was excluded from this study because its small number of samples is not appropriate for building of prediction models. The data that this study uses include architectural smells detected in recovered architectures, implementation issues collected from the Jira issue repository \cite{jiraclient}, and code commits extracted from GitHub \cite{github}. 

\begin{comment}
\bgroup
\def\arraystretch{1.25}
\begin{table}[bt]%[htbp]
	%\vspace{-3mm}
	\centering
	\caption{Subject systems used in building prediction models}
	%	\vspace{-2mm}
	\scriptsize
	%\resizebox{\columnwidth}{!} {
	\begin{tabular}{|l|p{3.5cm}|p{2.25cm}|p{2.25cm}|p{2.25cm}|}
		\toprule
		\textbf{System} & \textbf{Domain}   & {\textbf{\# Versions}} & \textbf{\# Issues} & \textbf{Avg. LOC} \\
		\midrule
		%ActiveMQ    & Messaging Framework    & 45             & 5583      & 1.65M \\
		Camel       & Integration F-work  & 78             & 9665      & 1.13M \\ 
		%Continuum   & Integration Server     & 11             & 2312      & 463K  \\
		CXF         & Service F-work      & 120            & 6371      & 915K  \\
		Hadoop      & Data Proc. F-work & 63             & 9381      & 1.96M \\
		%Ivy   		& Dependency Manager 	 & 20    		  &  		  & 400K \\
		%	Log4J       & Logging Framework      & 38             & 754       & 257K  \\
		%	Lucene      & Search Engine          & 52             & 6047      & 558K  \\
		Nutch       & Web Crawler      		 & 21             &	1928	      & 118K  \\
		OpenJPA		& Java Persist. 	 	 & 20    		  & 1937 	  & 511K \\
		Struts2     & Web App F-work      & 36             & 4207      & 379K  \\
		%	Openjpa     & Java EE Persistence    & 23             & 1908      & 508K  \\
		Wicket      & Web App F-work      & 72             & 6098      & 332K  \\
		%	\midrule
		%	\textbf{Total} &  & \textbf{}    & \textbf{} & \textbf{} \\
		\bottomrule
	\end{tabular}%
	\vspace{1.5mm}
	\label{tab:subject_systems_predict}%
\end{table}%
\egroup
\end{comment}

%These information will be used to tie the properties of a system's implementation and its underlying architecture to the likelihood of issues and changes. This will be accomplished via a novel technique and accompanying tools that comprise necessary software analyses. 

\section{Results}

For each research question, the method employed in validating it and the associated findings will be discussed in the following sections.

\subsection{RQ1. To what extent can the architectural smells detected in a system help to predict the issue-proneness and change-proneness of that system at a given point in time?}

\begin{table*}[bth]
	\centering
	\caption{Predicting Issue-proneness using Decision Table}
	\label{RQ1.issues_proneness}
	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{System} & \multicolumn{3}{c|}{ACDC}    & \multicolumn{3}{c|}{ARC}     & \multicolumn{3}{c|}{PKG}     \\ \cline{2-10} 
		& Precision & Recall & F-score & Precision & Recall & F-score & Precision & Recall & F-score \\ \hline
		Camel & 69.9\%    & 68.4\% & 68.9\%  & 70.8\%    & 67.0\% & 67.5\%  & 68.2\%    & 62.8\% & 63.4\%  \\ \hline
		CXF                     & 78.0\%    & 76.7\% & 77.1\%  & 68.9\%    & 68.3\% & 68.3\%  & 64.7\%    & 63.8\% & 63.8\%  \\ \hline
		Hadoop                  & 81.2\%    & 80.1\% & 80.3\%  & 76.6\%    & 76.6\% & 75.4\%  & 72.8\%    & 73.4\% & 72.1\%    \\ \hline
		Nutch                   & 80.8\%    & 71.6\% & 70.9\%  & 82.5\%    & 82.7\% & 82.3\%  & 68.3\%    & 52.1\% & 43.7\%  \\ \hline
		OpenJPA                 & 71.4\%    & 68.3\% & 70.8\%  & 74.5\%    & 73.2\% & 72.6\%  & 69.2\%    & 67.9\% & 67.3\%  \\ \hline
		Struts2                  & 89.2\%    & 89.0\% & 89.0\%  & 95.0\%    & 94.8\% & 94.8\%  & 79.1\%    & 78.3\% & 78.4\%  \\ \hline
		Wicket                  & 69.2\%    & 70.1\% & 68.8\%  & 76.7\%    & 77.1\% & 76.5\%  & 63.7\%    & 65.4\% & 59.6\%  \\ \hline
		Average                  & 77.1\%    & 74.9\% & 75.1\%  & 77.9\%    & 77.1\% & 76.8\%  & 69.4\%    & 66.2\% & 64.0\%  \\ \hline
	\end{tabular}
\end{table*}

In our prediction problem, all the features are binary (recall Table \ref{tab:data_point_sample}). A feature indicates whether or not a file has an architectural smell.
For this reason, decision-based techniques are likely to yield a better result than others. Our observation of the evaluation metrics yielded by different classification techniques --- such as decision table \cite{kohavi1995power}, decision tree \cite{quinlan2014c4}, logistic regression \cite{le1992ridge}, naive bayes \cite{john1995estimating} --- also confirms this intuition. 
%Tables \ref{RQ1.issues_proneness} 
This section will only discuss the obtained results of % precisions, recalls and f-scores of issue-proneness
the decision table based models, which %based on the decision table technique. This technique 
generally has the best accuracy among the aforementioned prediction techniques.  %The numbers in the result tables are weighted precision, recall and f-score, which are computed by WEKA. 

Table \ref{RQ1.issues_proneness} shows the precisions, recalls and f-scores of the decision table models for predicting the issue-proneness of 7 subject systems. Those values are computed using the 10-fold-cross-validation setup \cite{kohavi1995study}. The left column shows the systems' name and the last row shows the average values across all the systems. 
For each system, we built three different prediction models based on three sets of architectural smells, which were detected in three architectural views: ACDC, ARC, and PKG. In total, 21 prediction models based on the decision table technique were created and evaluated. 

In general, the prediction models of PKG yield the lowest accuracy. The models of ACDC and ARC %\rhl{
exhibit performance that is up to 15\% better than PKG. %} 
Across all the systems, the prediction models of ACDC achieve the precision of at least 69.2\%, the recall of at least 68.4\%, and f-score of at least 68.8\%. The corresponding values of the prediction models of ARC are 68.9\%, 67.0\%, and 67.5\%. Notably, the prediction model of Struts2 under ARC view achieves $\sim$95.0\% in all three metrics. 
As a result, ARC has the highest average accuracy, which is 77.9\% in precision, 77.1\% in recall, and 76.8\% in f-score. The corresponding values in ACDC are slightly lower, 77.1\% in precision, 74.9\% in recall, and 75.1\% in f-score. 

%\rhl{
These results confirm that architectural smell-based models can accurately predict the issue-proneness of a system. In other words, architectural smells have a consistent impact on a system's implementation with respect to issue-proneness over the system's lifetime. This finding will provide software maintainers with a powerful indicator of an implementation's health. %, which is architectural smells. 
It urges the maintainers to pay more attention to architectural smells existed in their systems. The maintainers can use the architectural smell-based prediction models to foresee future problems as well as to devise refactoring plans. 


The relatively poor performance of PKG in answering RQ1 is in line with one finding that emerged from our first empirical study on architectural changes (recall Chapter \ref{sec:empirical_change}). The finding showed that PKG is not as useful for software architects as ACDC and ARC, in order to understand the actual underlying architectural changes. In this study, PKG again shows that is not as useful as ACDC and ARC in correctly capturing the impact of the underlying architectural smells. This can be explained by the fact that PKG is a simple architecture recovery technique which only depends on the package structure of subject systems. On the other hand, ACDC and ARC do clustering based on sophisticated algorithms with respect to the systems' dependencies and concerns. Recall the categorization of architectural smells in Chapter \ref{sec:smells_detection}: two categories out of the four are dependency-based and concern-based smells. This observation suggests a future work for us to examine whether a smell should be detected under a specific architectural view in order to be more accurate.
%}


\begin{table*}[t]
	\centering
	\caption{Predicting Change-proneness using Decision Table}
	\label{RQ1.change_proneness}
	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{System} & \multicolumn{3}{c|}{ACDC}                                                                   & \multicolumn{3}{c|}{ARC}                                                                    & \multicolumn{3}{c|}{PKG}                                                                    \\ \cline{2-10} 
		& \multicolumn{1}{l|}{Precision} & \multicolumn{1}{l|}{Recall} & \multicolumn{1}{l|}{F-score} & \multicolumn{1}{l|}{Precision} & \multicolumn{1}{l|}{Recall} & \multicolumn{1}{l|}{F-score} & \multicolumn{1}{l|}{Precision} & \multicolumn{1}{l|}{Recall} & \multicolumn{1}{l|}{F-score} \\ \hline
		Camel                   & 69.9\%                         & 63.4\%                      & 63.3\%                       & 68.0\%                         & 67.1\%                      & 63.2\%                       & 60.3\%                         & 61.0\%                      & 61.9\%                       \\ \hline
		CXF                     & 73.7\%                         & 70.8\%                      & 78.3\%                       & 69.7\%                         & 63.4\%                      & 64.1\%                       & 60.8\%                         & 63.4\%                      & 62.8\%                       \\ \hline
		Hadoop                  & 78.1\%                         & 73.2\%                      & 75.6\%                       & 74.9\%                         & 74.8\%                      & 73.7\%						& 67.4\%                         & 70.0\%                      & 68.2\%                       \\ \hline
		Nutch                   & 73.1\%                         & 66.8\%                      & 67.9\%                       & 76.3\%                         & 78.0\%                      & 82.0\%                       & 62.2\%                         & 46.1\%                      & 44.7\%                       \\ \hline
		OpenJPA                 & 78.3\%                         & 77.7\%                      & 73.0\%                       & 74.3\%                         & 70.0\%                      & 66.5\%                       & 68.2\%                         & 62.1\%                      & 64.4\%                       \\ \hline
		Struts2                  & 89.3\%                         & 85.8\%                      & 83.1\%                       & 87.8\%                         & 96.7\%                      & 96.0\%                       & 71.2\%                         & 73.7\%                      & 80.2\%                       \\ \hline
		Wicket                  & 66.6\%                         & 65.3\%                      & 65.9\%                       & 72.1\%                         & 71.8\%                      & 73.3\%                       & 62.7\%                         & 59.0\%                      & 56.4\%                       \\ \hline
		Average        & 75.4\%                         & 72.7\%                      & 73.3\%                       & 74.7\%                         & 74.5\%                      & 74.1\%                       & 64.7\%                         & 62.2\%                      & 62.7\%  \\ \hline
		
	\end{tabular}
\end{table*}

Like issue-proneness, we used the same approach to evaluate the accuracy of 21 architectural smell based models for predicting change-proneness. Table \ref{RQ1.change_proneness} shows the accuracy of models built using the decision table technique. The models of PKG again have the lowest accuracy. In some systems like CXF, Nutch, and Struts2, the evaluation values in PKG are 10-20\% lower than the corresponding values in the other two views. This is similar to the result of issue-proneness.  
In the ACDC view, the average precision is 75.4\%, the average recall is 72.7\%, and the average f-score is 73.3\%. The corresponing numbers in the ARC views are 74.7\%, 74.5\% and 74.1\%.
%the precisions are at least 66.6\%, the recalls are at least 65.3\% and the f-score are at least 65.9\%. The corresponding values in the ARC view are 67.4\%, 63.4\% and 63.2\%. In many cases, the accuracy metrics are from 80-90\% or higher. 
%On average, the models of ACDC has slightly higher accuracy higher than ARC, between 72.7\% and 75.4\%.
These results again are promising and they prove that architectural smells based models can accurately predict the change-proneness of a system. 

%\rhl{
In summary, we can use the historical data of a system regarding its architectural smells, issues, and changes %of a system 
to develop the models which can predict issue- and change-proneness of that system with high accuracy. This result indicates that architectural smells have a consistent impact on systems' implementations. 
Our architecture-based prediction approach is useful for maintainers to foresee likely future problems in newly smell-impacted parts of the system. The approach could also help in creating maintenance plans in order to effectively reduce the system's issue- and change-proneness. Lastly, ACDC and ARC outperform PKG in predicting both issue- and change-proneness. This again emphasizes the importance of architectural recovery techniques to help developers understand the underlying architecture precisely. %The result also suggested a future work, in which we would like to validate if architectural smells should be detected under a specific architectural view to get the highest accuracy. 
% }

\subsection{RQ2. To what extent do unrelated software systems tend to share properties with respect to issue- and change-proneness?}

The results of the RQ1-related experiments show that architectural smells have consistent impacts on the issue- and change-proneness of a software system during its lifetime. In that sense, the RQ2 can be considered as an extension of the RQ1, in which we would like to see if architectural smells have consistent impacts across unrelated software systems. Specifically, we would like to see if the issue- and change-proneness of a system can be accurately predicted by the models trained by data from other unrelated software systems. 

To answer this research question, instead of using 10-fold-cross-validation, we sequentiality select a system from seven subject systems as the test system and use its dataset as the test set. The training set is created by combining datasets of other systems. To obtain comprehensive results, we conducted different experiments by combining six, five, and four systems (excluding the test system). If we select the other six systems, there is only one combination. However, if we select five out of the six systems, there are six different combinations. We tried all those six combinations and computed the means %and standard deviation 
of precisions and recalls. Similarly, for combining four out of the six systems, we tried all fifteen possible combinations and computed the mean and standard deviation of precisions and recalls. %\rhl{
Note that the datasets of different subject systems have different sizes, hence we have to resample those datasets to a same size before combining them.%}

%As ACDC has the highest result in the RQ1, we particularly focuses on the result of the RQ2 under ACDC view. 
Tables \ref{tab:rq2_all_data}, \ref{tab:rq2_all_data_arc}, and \ref{tab:rq2_all_data_pkg} summarize the results of all RQ2-related experiments with regard to predicting issue-proneness under ACDC, ARC, and PKG, respectively. The left sides of these tables show the list of systems. The precisions and recalls in 5 different cases are presented: 10-fold-cross-validation (``10-fold'' column) on the test test, models trained by 7 datasets including the test set (``All 7'' column), models trained by 6 other systems' datasets (``6 Others'' column), models trained by 5 other systems' datasets (``5 Others'' column), and models trained by 4 other systems' datasets (``4 Others'' column). Note that the "5 Others" and "4 Others" columns contain the mean values of the evaluation metrics of the models  %in all the possible %cases.%of 
which are trained on all possible combinations of systems. %\rhl{
In summary, beside 21 issue-proneness models from the RQ1's experiments, we built and evaluated 483 more issue-proneness models to answer the RQ2.%}  

%\rhl{
We found consistent trends in all three architectural views. First, a prediction model built by combining datasets of different software systems, even if the test system is included, has lower precision and recall than the model built for that specific test system. In all three Tables  \ref{tab:rq2_all_data}, \ref{tab:rq2_all_data_arc}, and \ref{tab:rq2_all_data_pkg}, the ``10-fold'' columns have the highest precision and recall values. %in both precision and recall. 
This result can be explained by the intuition that adding more systems' datasets can create a more general-purpose model, but it also adds noise and reduces the model's capability in predicting the properties of a specific system. %}
For this reason, if the dataset of a system is available, its prediction models should be trained only on its own dataset. 

Second, the prediction models trained by the datasets of six systems---excluding the test system--- yield relatively high precisions and recalls. They are close to their corresponding values in ``All 7'' columns, %\rhl{
and lower than corresponding values in the ``10-fold'' columns by $\sim$10\% or less.%}
For example, for the models built by 6 systems under the ACDC view (Table \ref{tab:rq2_all_data}), the precisions are from 63.4\% to 85.3\% and the recalls are from 56.5\% to 83.2\%. %\rhl{
Similarly, the prediction models trained by the datasets of 5 systems also achieve good results. Notably, in some cases, the results in ``5 Others'' are equal or slightly higher the corresponding values in ``6 Others''. Especially in the ARC view, precision values in "5 Others" columns are slightly higher than the ones in "6 Others" for all the systems, and  recall values in "5 Others" columns are slight higher than the ones in "6 Others" for five of seven systems. This observation shows that using a very large number of systems to train the model might slightly reduce the prediction models' accuracy because the models become too generic.%} 


\begin{table}[tb]
	\centering
	\caption{Predicting issue-proneness using the datasets of other subject systems - ACDC view}
	\label{tab:rq2_all_data}
	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{System} & \multicolumn{5}{c|}{Precision}                                                                 & \multicolumn{5}{c|}{Recall}                                                                    \\ \cline{2-11}
		& 10-fold & All 7 & 6 Others  & 5 Others & 4 Others & 10-fold & All 7 & 6 Others & 5 Others & 4  Others \\ \hline
		Camel   & 69.9\%                   & 63.7\%        & 63.5\%          & 61.7\%          & 43.9\%          & 63.4\%                   & 56.6\%        & 56.5\%          & 56.4\%          & 44.2\%          \\ \hline
		CXF     & 78.0\%                   & 77.1\%        & 75.1\%          & 74.7\%          & 50.0\%          & 76.7\%                   & 73.2\%        & 71.7\%          & 71.3\%          & 43.3\%          \\ \hline
		Hadoop  & 81.2\%                   & 74.8\%        & 69.8\%          & 70.0\%          & 41.3\%          & 80.4\%                   & 73.5\%        & 69.9\%          & 70.0\%          & 42.1\%          \\ \hline
		Nutch   & 84.1\%                   & 74.9\%        & 74.9\%          & 74.9\%          & 41.6\%          & 77.3\%                   & 68.8\%        & 68.8\%          & 68.8\%          & 40.4\%          \\ \hline
		OpenJPA & 71.4\%                   & 66.7\%        & 65.1\%          & 65.3\%          & 49.9\%          & 68.3\%                   & 63.9\%        & 62.0\%          & 62.3\%          & 49.9\%          \\ \hline	
		Struts2  & 89.2\%                   & 85.3\%        & 83.1\%          & 82.6\%          & 48.8\%          & 89.0\%                   & 85.4\%        & 83.2\%          & 82.7\%          & 43.1\%          \\ \hline
		Wicket  & 69.2\%                   & 63.4\%        & 63.4\%          & 60.1\%          & 48.2\%          & 70.1\%                   & 64.6\%        & 64.6\%          & 61.5\%          & 52.9\%          \\ \hline
	\end{tabular}
\end{table}

\begin{table}[b]
	\centering
	\caption{Predicting issue-proneness using the datasets of other subject systems - ARC view}
	\label{tab:rq2_all_data_arc}
	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{System} & \multicolumn{5}{c|}{Precision}                                                                 & \multicolumn{5}{c|}{Recall}                                                                    \\ \cline{2-11}
		& 10-fold & All 7 & 6 Others  & 5 Others & 4 Others & 10-fold & All 7 & 6 Others & 5 Others & 4  Others \\ \hline
		Camel   & 70.8\% & 68.1\% & 63.6\% & 63.7\% & 38.1\% & 67.0\% & 61.2\% & 59.9\% & 59.6\% & 37.1\% \\ \hline
		Cxf     & 68.9\% & 62.1\% & 58.0\% & 58.2\% & 45.4\% & 68.3\% & 59.5\% & 55.3\% & 55.0\% & 43.7\% \\ \hline
		Hadoop  & 72.8\% & 75.3\% & 73.7\% & 74.1\% & 38.2\% & 73.4\% & 74.9\% & 70.1\% & 70.4\% & 38.5\% \\ \hline
		Nutch   & 82.5\% & 86.9\% & 81.8\% & 82.3\% & 31.3\% & 82.7\% & 84.1\% & 78.1\% & 79.2\% & 38.2\% \\ \hline
		OpenJPA & 74.5\% & 71.2\% & 69.0\% & 69.9\% & 32.7\% & 73.2\% & 69.7\% & 67.1\% & 67.7\% & 38.9\% \\ \hline
		Struts2 & 95.0\% & 92.9\% & 91.8\% & 92.1\% & 34.8\% & 94.8\% & 92.5\% & 91.5\% & 91.9\% & 38.8\% \\ \hline
		Wicket  & 76.7\% & 65.6\% & 64.7\% & 64.9\% & 34.4\% & 77.1\% & 65.9\% & 65.2\% & 65.3\% & 39.0\% \\ \hline
	\end{tabular}
\end{table}

\begin{table}[tb]
	\centering
	\caption{Predicting issue-proneness using the datasets of other subject systems - PKG view}
	\label{tab:rq2_all_data_pkg}
	\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multirow{2}{*}{System} & \multicolumn{5}{c|}{Precision}                                                                 & \multicolumn{5}{c|}{Recall}                                                                    \\ \cline{2-11}
		& 10-fold & All 7 & 6 Others  & 5 Others & 4 Others & 10-fold & All 7 & 6 Others & 5 Others & 4  Others \\ \hline
		Camel   & 68.2\% & 66.0\% & 64.8\% & 64.7\% & 52.0\% & 62.8\% & 59.6\% & 59.2\% & 59.0\% & 45.2\% \\ \hline
		Cxf     & 64.7\% & 53.6\% & 52.3\% & 52.6\% & 45.9\% & 63.8\% & 50.7\% & 46.6\% & 47.6\% & 43.7\% \\ \hline
		Hadoop  & 76.6\% & 71.6\% & 69.9\% & 70.1\% & 38.6\% & 76.6\% & 69.6\% & 68.1\% & 68.3\% & 39.4\% \\ \hline
		Nutch   & 68.3\% & 64.6\% & 63.1\% & 63.6\% & 56.5\% & 52.1\% & 48.1\% & 45.2\% & 46.1\% & 41.6\% \\ \hline
		OpenJPA & 69.2\% & 66.7\% & 65.6\% & 65.7\% & 40.5\% & 67.9\% & 66.1\% & 64.9\% & 65.0\% & 42.4\% \\ \hline
		Struts2 & 79.1\% & 77.7\% & 74.5\% & 74.9\% & 54.3\% & 78.3\% & 77.5\% & 73.9\% & 74.4\% & 53.7\% \\ \hline
		Wicket  & 63.7\% & 63.7\% & 63.2\% & 62.5\% & 52.2\% & 65.4\% & 65.4\% & 65.2\% & 64.2\% & 52.6\% \\ \hline
	\end{tabular}
\end{table}

The third observations is that the precisions and recalls of the prediction models are reduced significantly when the number of training systems is reduced to four. %\rhl{
In most of the cases of all three architectural views, the precisions and recalls in ``4 Others'' columns are lower than corresponding values in ``5 Others'' columns by at least $\sim$15\% or more. %} 
It suggests that combining four systems is not enough to build a generic prediction model, if that model is intended to be used on unrelated systems.

Tables \ref{tab:5_systems} and \ref{tab:4_systems} show the further details of our experiments with the combinations of five and four systems, respectively, under the ACDC view. 
As mentioned in the beginning of this section, for each test system, there are six possible combinations of five other systems' datasets, and fifteen possible combinations of four other systems' datasets. Tables \ref{tab:5_systems} and \ref{tab:4_systems} show the means and the standard deviations of both the precisions and recalls for each test system. %\rhl{
%A mean is the average of a set of data values. A standard deviation is the measurement to quantify the amount of variation of that set. A low standard deviation indicates that the data values tend to be close to the mean, while a high standard deviation indicates that the data values are spread out over a wider range around the mean. %}
The tables show that the combinations of five systems not only have the high means of precisions and recalls but also have the low standard deviations of both precisions and recalls. %\rhl{
The standard variations of precisions and recalls are less than 5\% when we combine five systems.  
In contrast, the combinations of four systems have the low means and high standard deviations of those two metrics. %and the high standard deviations of those two metrics
The standard variations of precisions and recalls can go up to 10\% in this case. 
A low standard deviation indicates that the data values tend to be close to the mean, while a high standard deviation indicates that the data values are spread out over a wider range around the mean.
These results indicate that the accuracy of prediction models starts converging while we increase the number of systems in the training sets. The more systems we includes, the lower variation is, until the accuracy reaches its maximum vales. Based on our experiments, combining five systems generally yields the best results.%}



\begin{table}[tb]
	\centering
	\caption{Predicting issue-proneness using combinations of 5 other systems}
	\label{tab:5_systems}
	\begin{tabular}{|l|c|c|c|c|}
		\hline
		\multirow{2}{*}{System} & \multicolumn{2}{c|}{Precision} & \multicolumn{2}{c|}{Recall} \\ \cline{2-5} 
		& Mean       & Std. Dev.     & Mean      & Std. Dev.   \\ \hline
		Camel                   & 61.7\%     & 5.0\%             & 66.4\%    & 1.0\%           \\ \hline
		CXF                     & 74.7\%     & 2.3\%             & 71.3\%    & 1.7\%           \\ \hline
		Hadoop                  & 70.0\%     & 0.4\%             & 70.0\%    & 0.3\%           \\ \hline
		Nutch                   & 74.9\%     & 0.0\%             & 68.8\%    & 0.0\%           \\ \hline
		OpenJPA                 & 65.3\%     & 0.4\%             & 62.3\%    & 0.5\%           \\ \hline
		Struts2                  & 82.6\%     & 1.5\%             & 82.7\%    & 1.5\%           \\ \hline
		Wicket                  & 60.1\%     & 4.0\%             & 61.5\%    & 3.5\%           \\ \hline
	\end{tabular}
\end{table}


\begin{table}[tb]
	\centering
	\caption{Predicting issue-proneness using combinations of 4 other systems}
	\label{tab:4_systems}
	\begin{tabular}{|l|c|c|c|c|}
		\hline
		\multirow{2}{*}{System} & \multicolumn{2}{c|}{Precision} & \multicolumn{2}{c|}{Recall} \\ \cline{2-5} 
		& Mean       & Std. Dev.     & Mean      & Std. Dev.   \\ \hline
		Camel                   & 43.9\%     & 8.8\%             & 44.2\%    & 3.8\%           \\ \hline	
		CXF                     & 50.0\%     & 8.5\%             & 43.3\%    & 3.8\%           \\ \hline
		Hadoop                  & 41.3\%     & 8.1\%             & 42.1\%    & 9.3\%           \\ \hline
		Nutch                   & 41.6\%     & 7.1\%             & 40.4\%    & 5.9\%           \\ \hline
		OpenJPA                 & 49.9\%     & 4.9\%             & 49.9\%    & 2.7\%           \\ \hline
		Struts2                  & 48.8\%     & 10.0\%            & 43.1\%    & 9.3\%           \\ \hline
		Wicket                  & 48.2\%     & 7.5\%             & 52.9\%    & 3.6\%           \\ \hline
		
	\end{tabular}
\end{table}

We also found the similar trends in the experiments which attempt to predict the change-proneness of a system using unrelated systems' datasets. %\rhl{
In summary, the results of the RQ2-related experiments confirm that software systems tend to share properties with respect to issue- and change-proneness. 
The accuracy of generic models is less than the one of specific models, however, the gap is just about 10\% or less. 
This allows developers to use generic models to predict the issue- and change-proneness of new software systems in the early stages of their development, before sufficiently large numbers of system versions become available.
Furthermore, our empirical study's results suggest that using at least five systems can create a reliable generic model which can predict the issue- and change-proneness of new software systems with high accuracy. %As one of our future works, we would like to extend the number of subject systems to firmly verify our findings.%}


==> arch_concepts_formalization.tex <==
%\vspace{-3mm}
\subsection{Formalization of Architectural Concepts}
\label{subsec:smells_concepts}

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.45]{graphics/simple_arch.pdf}
	\vspace{-6mm}
	\caption{A notional software system's architecture. }
	\label{fig:simple_arch}
\end{figure}


%\subsubsection{Architecture}

Figure \ref{fig:simple_arch} shows a notional software architecture $A$ that comprises two components, $C_1$ and $C_2$. Each component contains multiple implementation-level entities. Between entities, links are presented by solid arrows and couplings by dashed lines. %For the rest of this section, we will formalize these concepts and the relationships between them.
In the view of typical recovery methods %employed here and a number of others 
 \cite{garcia2013obtaining}, we represent the  structure of a system's architecture as a graph \textit{A} whose vertices represent the system's components \textit{C} and  topology represents the connections embodied in the set of links \textit{L} and the set of couplings \textit{Cp} between these components: $A = (\mathit{C}, \mathit{L}, \mathit{Cp})$

%\vspace{-1mm}
%\begin{noindent}
%\begin{center}
%\begin{tabular}{ll}
%$A = (\mathit{C}, \mathit{L}, \mathit{Cp})$\\
%\end{tabular}
%\end{center}
%\end{noindent}
%\vspace{-1mm}

%\subsubsection{System}
%In order to represent and detect concern-based smells, we model 
%\neno{We need a better characterization of a system and/or a proper characterization of what a system is more generally...} \daniel{This definition of "system" only applies to ARC. I suggest we move it to the architecture section and describe it in the context of ARC.}

%\rhl{A recovery method creates an architectural view based on what it deems the relevant parts of the system to come up with such its particular view\arman{this sentence is not clear}. The above formalization is based on well-accepted basic elements of software architecture. In our study, we 

Since our study involves a concern-based recovery technique (ARC),  we will also formalize this concept. For our purposes, the architecture of a software system %is a tuple that consists of architecture \textit{A}, which describes how the system's component communicate, and 
	can be associated with a nonempty set of topics \textit{T}, which captures functionalities of the system and its components. 
%\textit{T} can be obtained by using a topic modeling technique, such as LDA. 
We define a topic as a probability distribution \textit{Pd} over the system's nonempty set of keywords \textit{W}, whose elements are used to ``describe'' that system (e.g., via comments in source code). % modeled by the architecture. 
By examining the words that have the highest probabilities in a topic, the meaning of that topic may be discerned. %\daniel{Are we doing this? We've never done this to my knowledge.} \duc{No, we didn't do this. This is just a suggestion about how to understand topics.} 
In this way, a topic can serve as a representation of a \emph{concern} % (i.e., a concept, role, or responsibility) 
addressed by a system. The set of topics \textit{T} is then a representation of the system's concerns. 

\vspace{-2mm}
\begin{noindent}
	\begin{center}
		\begin{tabular}{l}
			%$\mathit{S} = (A,T)$ ~ %~~~~~~~ \\
			$W=\{w_i \mid i \in \mathbb{N}\}$ ~
			$T = \{z_i \mid i \in \mathbb{N} \}$ ~
			$z = Pd(W)$\\
		\end{tabular}
	\end{center}
\end{noindent}
\vspace{-2mm}

%A component can be  simple or composite.  A composite component is an architecture in its own right, allowing for multiple levels of architectural abstraction. Its definition is therefore the same as that for architecture \textit{A} above. %Our definition of architectural smells does not depend on architectural hierarchy, 
%Most of the automated architecture-recovery techniques \cite{garcia2013comparative} only recover the flattened %\yixue{flat?} 
%structure of software architecture (i.e., clustering entities into a set of components) and we thus exclude composite components from our formalization. \ducdelete{Additionally, since those recovery techniques overwhelmingly focus on components, we do not distinguish between components and connectors here.} %in our formalization and instead uniformly represent them as architectural components.

A component is a tuple comprising the component's internal entities \textit{E} and the probability distribution \textit{$\theta$} over the system's topics \textit{T}. Entities are implementation elements used to build a system. An entity e contains its interface $\mathit{I}$, % (a set of elements $ie$ that expose that component's functionality or data), 
a set of links $\mathit{L_E}$, and a set of couplings $\mathit{Cp_E}$ to other entities. In  OO systems, entities are classes and interfaces are public methods. % (and/or implemented interfaces) \daniel{Not seeing the need to mention implemented interfaces - those will just result in public methods, which are already mentioned} which allow interactions among classes. %, set of operations $\mathit{O}$, the map \textit{M} that relates the operations to the interfaces through which they are exported.

\vspace{-1mm}
\begin{center}
\begin{tabular}{ll}
%$\mathit{C} = \mathit{SC} \cup \mathit{CC}$ ~~~~~~~
$\mathit{C} = \{c_i \mid i \in \mathbb{N}\}$ ~~ 
$c = (E, \theta_c)$ ~~ \\
$\mathit{E} = \{e_i \mid i \in \mathbb{N}\}$ ~~ 
%$e = (I, O, M)$ ~~
$e_i = (I_i, L_{e_i}, Cp_{e_i})$ ~~
$\mathit{I} = \{ie_i \mid i \in \mathbb{N} \}$\\
\end{tabular}
\end{center}
\vspace{-1mm}


Both a link $l$ and a coupling $cp$ consist of a source $src$ and a destination $dst$, which are  the components' internal entities involved in an interconnection. Links are \textit{unidirectional}, while couplings are \textit{bidirectional}. The union of the links of all entities is the set of links \textit{L} of the graph $A$. The union of the couplings of all entities is the set of couplings \textit{Cp} of the graph $A$. %In the following formalization, `e' stands for an entity in the system. 
 %When composing the two unions, we convert the entities \textit{dst} and \textit{src} to their parent components, so that $L$ and $Cp$ are links and couplings between components. 
%\vspace{-5mm}
\begin{noindent}
\begin{center}
\begin{tabular}{ll}
	~~$L = \cap_{i=1}^{n}L_{e_i}$~~~~~~$\mathit{L_e} = \{l_j \mid i \in \mathbb{N}_0\}$ ~~~~~~~$l = (src, dst)$ ~~ \\
	%~~$Cp_E = Co \cap Du $ 
	~~$Cp = \cap_{i=1}^{n}Cp_{e_i}$~~$\mathit{Cp_e} = \{cp_j \mid i \in \mathbb{N}_0\}$ ~~ 	$cp = (src, dst)$ ~~ \\
	
%	$src, dst \in \mathbb{I}$ 
\end{tabular}
\end{center}
\end{noindent}
\vspace{-1mm}




%\end{comment}


==> arch_smells_catalog.tex <==
%\vspace{-5mm}
\subsection{Smell Formalization and Detection Algorithms}
\label{subsec:formal_arch_smells}
%In this section, we categorize important architectural smells based on the aspects of software systems they impact. The idea of this categorization was briefly proposed in our recent work \cite{le2016architectural}, which suggests an approach for predicting bugs in a software system using architectural knowledge. The categorization we provide in this paper is much more detailed.

%\subsection{Determining Thresholds to Detect Smells}
%\label{subsec:detection_strategies}
One critical issue in smell detection is setting thresholds, i.e., defining the criteria that serve as indicators of smells. %Thresholds are criteria to classify a value as an outlier. %or not. 
We set thresholds by using Interquartile analysis \cite{tukey1977exploratory}, which is a widely used, efficient technique \cite{Lanza:2005:OMP:1076853} for detecting outliers (i.e., smells in our study) in a population without requiring it to have a normal probability distribution. %This method has been used widely to define software metrics .

In the Interquartile method, the lower quartile ($q_1$) is the $25^{th}$ percentile, and the upper quartile ($q_3$) is the $75^{th}$ percentile of the data. The interquartile range ($iqr$) is defined as the interval between $q_1$ and $q_3$. $q_1-(1.5*iqr)$ and $q_3+(1.5*iqr)$ are defined as “inner fences”, that mark off the "reasonable" values from the outliers \cite{Fenton:1998:SMR:580949}. In this section, we will use a shorthand function %\textbf{\textit{getLowThreshold()}} and 
\textbf{\textit{getHighThreshold()}}, which accepts a list of values and return %the low and 
the high value of the ``inner fences''.
%}

\begin{algorithm}[!t]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
	%	\algsmall
	\scriptsize
	\caption{\bcoalgname}
	\label{alg:detectbco}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of components, $T$: a set of system concerns}%, $\mathit{th_{z_b}}$: threshold for concern relevance}
	\KwOut{$\mathit{COsmells}: $ a set of \bco instances }
	
	$\mathit{COsmells} \leftarrow \emptyset$\;
	$\mathit{componentConcernCounts} \leftarrow$ initialize all brick concern counts to 0\;
	\For{$c \in C$}{ \label{alg:detectbco:count_topics:start}
		$T_c \leftarrow \mathit{getConcernsOfComponent(c)}$\;
		$\mathit{th_{z_c}} \leftarrow \mathit{getHighThreshold(P(T_c))}$\; \label{alg:detectbco:compute_threshold}
		\For{$z \in T_c$}{
			\If{$P(z \mid c) > \mathit{th_{z_c}}$} {
				$\mathit{componentConcernCounts}[c] = \mathit{componentConcernCounts}[c] + 1$\ \label{alg:detectbco:count_topics:end}
			}
		}
	}
	
	%$\mathit{meanBrickConcerns} \leftarrow \mathit{computeMean(brickConcernCounts)}$\; \label{alg:detectbco:mean}
	%$\mathit{stdDevOfBrickConcerns} \leftarrow \mathit{computeStandardDeviation(brickConcernCounts)}$\;\label{alg:detectbco:stddev}
	%$\mathit{th_{t}} \leftarrow \mathit{meanBrickConcerns} + \mathit{stdDevOfBrickConcerns}$
	
	$\mathit{th_{co}} \leftarrow \mathit{getHighThreshold(componentConcernCounts)}$\; \label{alg:detectbco:th_t}
	\For{$c \in C$}{ \label{alg:detectbco:detect:start}
		\If{$\mathit{componentConcernCounts[c]} > \mathit{th_{co}}$} {
			$\mathit{COsmells} \leftarrow \mathit{COsmells} \cup 
			\{c\}$\;\label{alg:detectbco:detect:end}
		}
	}
	
\end{algorithm}

\subsubsection{\textit{\underline{Concern Overload (CO)}}} indicates that a component implements an excessive number of concerns \cite{dijkstra1982role}. 
%CO is inspired by Stal's architectural smell called \textit{Component Responsibility Overload}~\cite{stal2011bqos}. While Stal uses the word ``responsibility,'' we use the word ``concern'' to mean the same here. 
CO %violates the principle of  separation of concerns \cite{dijkstra1982role}. It 
 may increase the size of a component, hurting its maintainability. 
%daniel{I would think the size and location of a component should also be taken into account. Consider a component that displays the main menu of a GUI-based application. Such a component will potentially address a lot of concerns, but it's not a problem.} \duc{In this case, I expect to see more keywords related to GUI (e.g., button, field) than other concerns. But I agree this case will cause confusion sometimes.}
Formally, a component $c$ % \in C$ 
suffers from this smell iff

~~~~~~~~$ |\; \{z_j \mid (j \in \mathbb{N}) \wedge (P(z_j \mid c) > th\_z_c) \} \;|  > th_{co}$

%\arman{sorry if I missed it, did we somewhere explain the N and $\mathbb{N}_0$. We are surely not checking for all the natural numbers here...}
\noindent where thresholds $0 \leq th\_z_c \leq 1$ and $th_{co} \in \mathbb{N}$, respectively, indicate   a topic is significantly represented in the component and the maximum acceptable number of concerns per component.  

%\vspace{-8mm}
Algorithm \ref{alg:detectbco}, \bcoalgname, determines which components in the system have CO. 
%The algorithm operates in a manner similar to \spfalgname. 
\bcoalgname begins by creating a map, $componentConcernCounts$, where keys are components and values are  numbers of relevant concerns in each component (Lines \ref{alg:detectbco:count_topics:start}-\ref{alg:detectbco:count_topics:end}). While creating the map, threshold $\mathit{th_{z_c}}$ is dynamically computed (Line \ref{alg:detectbco:compute_threshold}) and used to determine prevalent concerns for each component.\bcoalgname uses that map to compute threshold $th_{co}$ (Line  \ref{alg:detectbco:th_t}), which is then used to determine which components have the CO smell (Lines \ref{alg:detectbco:detect:start}-\ref{alg:detectbco:detect:end}).




\subsubsection{\textit{\underline{Dependency Cycle (DC)}}} indicates a set of components whose links form a circular chain, causing changes to one component to possibly affect all other components in the cycle. %Furthermore, {this smell may imply coupling between components. Specifically, } an issue occurring in one component may potentially propagate to all the other components in the cycle. 
Such high coupling between components violates the principle of modularity.
%\daniel{I would require some kind of "distance" between the components that makes it so they can't easily be joined (which would make the cycle go away). There may be cases where someone simply split up a large file into several small ones that reside in the same folder/package. They may then be strongly connected, but it's not as meaningful as it would be if they resided in different packages and have "roots" (i.e. lots of connections) in those.} \duc{I think in that cases, those files will be clustered in a same component by recovery techniques, then we do not consider them as DC because they are in a same component.}
Formally, this smell occurs in a set of three or more components iff %$\mathit{c_k \in DC}$ iff
%\begin{alloy}
%pred check_dc (DC: set Component) {
%	#(DC) > 3 && 
%	all c: DC | c in c.^(entities.out_link.parent)}
%\end{alloy}

~~~~~~$\exists l \in L \mid (\forall x \mid (1 \leq x \leq k) \mid \\
~~~~~~~~~~~~~((x < k) \implies \mathit{(l.src \in c_x.\mathit{E} \wedge l.dst \in c_{x+1}.\mathit{E})}) \wedge \\
~~~~~~~~~~~~~((x = k) \implies \mathit{(l.src \in c_x.\mathit{E} \wedge l.dst \in c_1.\mathit{E}))}  $

%\noindent
%where the predicate $\mathit{linked(c_i,c_j,l)}$ is true if $l.src = c_i \wedge l.tgt = c_j$. %We also define the set of paths in the architecture, $PT = \{pt_i \mid i \in \mathbb{N} \}$ and a function 
%The function $\mathit{compAtPos}_{pt_i}(pos) : \mathbb{N} \rightarrow C$ is defined for each $pt_i \in PT$ and returns the component at position $pos$ for path $pt_i$. 
%This smell occurs for dependency path $pt_j \in PT$ iff
%\noindent ~~~ $\exists pos_1,pos_2 \in \mathbb{N} \mid compAtpos_{pt_j}(pos_1) = compAtpos_{pt_j}(pos_2) \wedge pos_1 = 1 \wedge pos_2 = \mathit{len}(pt)$
%\noindent
%where $\mathit{len}(pt)$ is the length of $pt$. 

We detect DC smells by identifying \emph{strongly connected subgraphs} in a  system's architectural graph $G = (C,L)$. A strongly connected subgraph is one where each vertex is reachable from every other vertex. %Each strongly connected component in $G$ is a \bdc. 
Algorithms that detect strongly connected subgraphs are well known \cite{dijkstra1976discipline} %,leiserson2001introduction}
and can  be used to identify DC smells. %Therefore, we do not include the detection algorithm for DC in this paper. %\bdcs.

\subsubsection{\textit{\underline{Link Overload (LO)}}} is a dependency-based smell that occurs when a component has interfaces involved in an excessive number of links (e.g., call dependencies), affecting the system's separation of concerns and isolation of changes. % For example, modifications to a component with LO due to an excessive number of outgoing links can potentially affect every  component to which it is linked.
%Conversely, 
%any component with an excessive number of incoming links becomes brittle because it is affected by many other components.
\begin{comment}
\begin{table}[h]
\centering
\caption{\lo Variants}
\scriptsize
\begin{tabular}{ccc} 

\toprule
Link Type for Variant &$\mathit{direction(l)}$\\
\toprule

Incoming links& $l = (ie_2,ie_1)$ \\ \midrule
Outgoing links& $l = (ie_1,ie_2)$\\ \midrule
Both incoming and outgoing links& $l = (ie_1,ie_2) \vee l = (ie_2,ie_1)$\\ \bottomrule

\end{tabular}
\label{tab:lo_variation}
\end{table} 
\end{comment}
%A component may have an excessive number of incoming links, outgoing links, or both. Consequently, we define three variants of LO. 
Formally, a component $c$ suffers from both incoming and outgoing link overload iff


~~$|\, \{l \in L \mid l.src \in c.\mathit{E} \} \,| + |\, \{l \in De \mid l.dst \in c.\mathit{E} \} \,| > th_{\mathit{lo}}$


\noindent where $th_{\mathit{lo}}$ is a threshold indicating the maximum number of links for a component that is considered reasonable. %Excessive incoming links and  outgoing links are defined analogously. 

\begin{algorithm}[t]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
	%	\algsmall
	\scriptsize
	\caption{\loalgname}
	\label{alg:detectlo}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of components, $L$: links between components}
	\KwOut{$\mathit{LOsmells}: $ a set of \lo instances }
	
	$\mathit{LOsmells} \leftarrow \emptyset$\;
	$\mathit{numLinks} \leftarrow$ initialize map as empty\;
	$\mathit{directionality} \leftarrow \{``in",``out",``both"\}$\;
	
	\For{$c \in C$}{ \label{alg:detectlo:numlinks:start}
		\For{$d \in directionality$} {
			$numLinks[(c,d)] \leftarrow numLinks[(c,d)] + 
			\mathit{getNumLinks(c,d,L)}$\;\label{alg:detectlo:numlinks:end}
		}
	}
	
	\For{$d \in directionality$} { \label{alg:detectbco:th_lo:start}
		%	$\mathit{meanLinks[d]} \leftarrow 
		%	\mathit{computeMean(numLinks,d,B)}$\;\label{alg:detectlo:stats:start}
		%	$\mathit{stdDevLinks[d]} \leftarrow 
		%	\mathit{computeStandardDeviation(numLinks,d,B)}$\;
		%	$\mathit{th_{lo}[d]} \leftarrow \mathit{meanLinks[d]} + 
		%	\mathit{stdDevLinks[d]}$\;\label{alg:detectlo:stats:end}
		$\mathit{th_{lo}[d]} \leftarrow \mathit{getHighThreshold(numLinks,d)}$\; \label{alg:detectbco:th_lo:end}
	}
	
	\For{$c \in C$}{ \label{alg:detectlo:detect:start}
		\For{$d \in directionality$} {
			\If{$\mathit{getNumLinks(c,d,L)} > \mathit{th_{lo}[d]}$} {
				$\mathit{LOsmells} \leftarrow \mathit{LOsmells} \cup 
				\{(c,d)\}$\;\label{alg:detectlo:detect:end}
			}
		}
	}
	
\end{algorithm}

Algorithm \ref{alg:detectlo}, \loalgname, extracts the LO variants for a set of components $C$ by examining their links $L$. The algorithm 
first determines the number of incoming and outgoing links per component 
(Lines \ref{alg:detectlo:numlinks:start}-\ref{alg:detectlo:numlinks:end}). 
\loalgname sets the threshold $th_{\mathit{lo}}$ for each variant of LO
% by computing the thresholds $th_{lo}$ for incoming, outgoing, and combined links 
 (Lines \ref{alg:detectbco:th_lo:start}-\ref{alg:detectbco:th_lo:end}).
%\ref{alg:detectlo:stats:start}-\ref{alg:detectlo:stats:end}).
 Finally, \loalgname identifies each component and the directionality 
that indicates the variant of LO from which the component suffers  (Lines 
\ref{alg:detectlo:detect:start}-\ref{alg:detectlo:detect:end}).



\subsubsection{\textit{\underline{Unused Interface (UI)}}} is an interface of a system  entity that is linked to no other entities.
%In this case, we say the entity itself is unused. The unused entity might have been added by developers for future use. However, 
Including entities in a system without any associated use cases violates the principle of incremental development \cite{Fowler:1997:UDA:270005}. Having that unused entity adds unnecessary complexity to the component and the software system which, in turn, hinders  maintenance. 
Formally, a component $c \in C$ contains a UI smell in entity $e \in b.\mathit{E}$ iff

%\noindent ~~~~~~~~~$\not\exists b_2 \in B | (ie_2 \in b_2.\mathbb{I}) \wedge (b_1 \not\equiv b_2) $ 
%~~~~~~~~~~~~$\wedge (((ie_1, ie_2) \in L) \vee ((ie_2, ie_1) \in L))$

~~~~~~~~~~~~~$ (|e.I| \neq 0) \wedge (\not\exists l \in e.L ~|~  l.dst = e)$ 

%\textit{\underline{Unused Interface (UI)}} and \textit{\underline{Unused Component (UC):}}
%As we mentioned in Section \ref{subsec:formal_arch_smells}, UC is the extreme case of UI. 
Algorithm \ref{alg:detectui_ub}, \textbf{\uiubsalgname}, detects this %both of these 
smell. \textbf{\uiubsalgname} uses the set of links L to determine if an interface has been used. The algorithm checks every entity in each component (Lines \ref{alg:detectui_ub:numlinks:start}-\ref{alg:detectui_ub:numlinks:end}), and if an entity has a public interface but no link,  the entity and its parent component are added to the UI instances list. %Line \ref{alg:detectui_ub:checkub} uses a boolean flag, \textit{isUB}, to mark that a component does not have UC if at least one entity in the component does not have UI. Line \ref{alg:detectui_ub:addub} checks and adds UC instances to the smell list.


% Unused Interface + Unused Brick
%\vspace{-8mm}
\begin{algorithm}[h]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
	%	\algsmall
	\scriptsize
	\caption{\uiubsalgname}
	\label{alg:detectui_ub}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of bricks, $L$: links between components}
	\KwOut{$\mathit{UIsmells}: $ a set of Unused Interface instances }%, $\mathit{UCsmells}: $ a set of Unused Brick instances }
	
	$\mathit{UIsmells} \leftarrow \emptyset$, 
	$\mathit{UCsmells} \leftarrow \emptyset$\;
	
	\For{$c \in C$}{ \label{alg:detectui_ub:numlinks:start}
		%$isUC \leftarrow true$ \\
		\For{$e \in c.E$} {
			\If{$\mathit{getNumInterfaces(e.I)} > 0 \land getNumLinks(e.L)= 0$} {
				%\If{$getNumLinks(e.L)= 0$} {
					$\mathit{UIsmells} \leftarrow \mathit{UIsmells} \cup 
					\{(c,e)\}$\;
				} \label{alg:detectui_ub:numlinks:end}
				%\Else{
				%	$isUC \leftarrow false$ \label{alg:detectui_ub:checkub}
				%}
			%}
		}
		%\If{$isUC$} {
		%	$\mathit{UCsmells} \leftarrow \mathit{UCsmells} \cup 
		%	\{(c)\}$\; \label{alg:detectui_ub:addub}
		%}
	}
	
\end{algorithm}

\subsubsection{\textit{\underline{Sloppy Delegation (SD)}}} occurs when a component delegates to other components  functionality  it could have performed internally.
%\daniel{The problem with this is that it's very subjective. The practicalities of programming can also result in situations where this makes sense, e.g. when the "small amount of functionality" is very complex and covered by a different programmer.} \duc{I have a constrain (outcall(e2) = 0) in the formalization to ensure this} In particular, a component could perform that functionality itself if \rhl{the required functionality is encapsulated in a single entity of another component. That entity, in fact, should be moved to the component which uses it.} 
%all the data it needs to perform that functionality is part of that component's state. 
An example of SD is a component that manages all aspects of an aircraft's current velocity, fuel level, and altitude, but  passes that data to an entity in another component that solely calculates that aircraft's burn rate. Such inappropriate separation of concerns complicates the system's data- and control-flow which, in turn, impacts system maintenance. 
Formally, SD occurs between components $c_1, c_2 \in C$ iff 

~~$\exists l \in L ~|~  l.src = e_1 \in c_1.E \land l.dst = e_2 \in c_2.E \\ 
~~~~~~~~~~(outLink(e2) = 0) \wedge (inLink(e2) < th_{sd}) \wedge (c_1 \not\equiv c_2)\\
$
\noindent where \textit{outLink(e)} and \textit{inLink(e)} return the numbers of links from and to entity \textit{e}, respectively. Threshold $th_{sd}$ ensures entity $e_2$ is not a library-type entity. In a strict constraint, $th_{sd} = 2$, meaning that $e_2$'s functionality is only used by $e_1$.

Algorithm \ref{alg:detectsd}, \textbf{\sdsalgname}, requires a threshold $th_{sd}$, which defines the minimum number of in-links to consider a delegation appropriate. The algorithm checks every link in each entity (Lines \ref{alg:detectsd:numlinks:start}-\ref{alg:detectsd:numlinks:end}), and if a link has a \textit{dst} entity which satisfies the checking condition of SD%(defined in Section \ref{subsec:formal_arch_smells})
, then the \textit{dst} entity and its parent component are added to the list of SD instances (Line \ref{alg:detectsd:addsd}).

\begin{algorithm}[!h]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
	%	\algsmall
	\scriptsize
	\caption{\sdsalgname}
	\label{alg:detectsd}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of bricks, $L$: links between components,\\ ~~~~~~~~$\mathit{th_{sd}}$: threshold for relevance delegation}
	\KwOut{$\mathit{smells}: $ a set of Sloppy Delegation instances }
	
	$\mathit{smells} \leftarrow \emptyset$\;
	%	$\mathit{numCouplings} \leftarrow$ initialize map as empty\;
	%	$\mathit{types} \leftarrow \{``fo",``ls"\}$\;
	
	\For{$c_1 \in C$}{ \label{alg:detectsd:numlinks:start}
		\For{$e_1 \in c_1.E$} {
			\For{$l \in e_1.L$}{
				\If{$l.src=e_1$}{\label{alg:detectsd:numlinks:end}
					$e_2 \leftarrow l.dst$\;
					$c_2 \leftarrow getParent(e_2)$\;
					\If{$(e_1 \not\equiv e_2) \land (getOutLink(e_2)=0) \land (getInLink(e_2)  <th_{sd})$}{
						$\mathit{smells} \leftarrow \mathit{smells} \cup 
						\{((c_1,e_1),(c_2,e_2))\}$\;
					} \label{alg:detectsd:addsd}
				}
			}
		}
	}
	
\end{algorithm}

\subsubsection{\textit{\underline{Co-change Coupling (CC)}}} is a logical coupling that occurs when changes to an entity of a given component also  require changes to an entity in another component. %(recall Section~\ref{sec:related_work}). CC has similar negative consequences to DF. 
%Specifically, making a single change to a system affected by CC smells might require engineers to check and make changes to multiple components each time.
Formally, a component $c \in C$ has a CC iff 

~~~~~~~~~~~~~~~~~$e_i \in c.E  ~|~  \sum_{i=1}^{n} |e_i.\mathit{Cp}| > th_{cc}$

\noindent where $th_{cc}$ specifies a threshold for an excessively high number of logical couplings.

%Detecting coupling-based smells is similar to detecting LO. The difference is that the detection algorithms use couplings instead of links as their input. %Detecting DF depends on \textit{duplicates}, and 
%Detecting CC depends on \textit{co-changes}. 
Algorithm \ref{alg:detectdf_cc}, \dfccalgname, shows how to detect this type of smell. %these two types of smells. 
The algorithm first creates a map between components and their total numbers of co-changes (Lines \ref{alg:detectdf_cc:numCouplings:start}-\ref{alg:detectdf_cc:numCouplings:end}). The $getNumCp$ function returns the number of co-changes of an entity.
\dfccalgname uses these maps to compute a threshold, $th_{cc}$, which is the high inner-fence value (Line %s \ref{alg:detectdf_cc:computedf}-
\ref{alg:detectdf_cc:computecc}). Finally, the algorithm visits each component again, checks, and adds detected smell instances into the smell list (Lines \ref{alg:detectdf_cc:detect:start}-\ref{alg:detectdf_cc:detect:end}).

\begin{algorithm}[h]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
	%	\algsmall
	\scriptsize
	\caption{\dfccalgname}
	\label{alg:detectdf_cc}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of bricks, $Cp$: couplings between components}
	\KwOut{%$\mathit{DFsmells}: $ a set of Duplicate Functionality , 
		$\mathit{CCsmells}: $a set of Co-change Coupling instances }
	
	%$\mathit{DFsmells} \leftarrow \emptyset$, 	
	$\mathit{CCsmells} \leftarrow \emptyset$, \;
	%$\mathit{numDu} \leftarrow$ initialize map as empty\;
	$\mathit{numCp} \leftarrow$ initialize map as empty\;
	
	\For{$c \in C$}{ \label{alg:detectdf_cc:numCouplings:start}
		\For{$e \in c.E$} {
			%$numDu[c] \leftarrow numDu[c] + 
			%\mathit{getNumDu(c,e.Du)}$\;
			$numCp[c] \leftarrow numCp[c] + 
			\mathit{getNumCp(e.Cp)}$\;
		} \label{alg:detectdf_cc:numCouplings:end}
	}
	
	%$\mathit{th_{df}} \leftarrow \mathit{getHighThreshold(numDu,C)}$\label{alg:detectdf_cc:computedf}\; 
	$\mathit{th_{cc}} \leftarrow \mathit{getHighThreshold(numCp.values)}$\label{alg:detectdf_cc:computecc}\; 
	
	
	\For{$c \in C$}{ \label{alg:detectdf_cc:detect:start}
		%\If{$\mathit{numDu[c]} > \mathit{th_{df}}$} {
		%	$\mathit{DFsmells} \leftarrow \mathit{DFsmells} \cup 
		%	\{(c)\}$\;
		%}
		\If{$\mathit{numCp[c]} > \mathit{th_{cc}}$} {
			$\mathit{CCsmells} \leftarrow \mathit{CCsmells} \cup 
			\{(c)\}$\;
		} \label{alg:detectdf_cc:detect:end}
	}
	
\end{algorithm}




==> discussion.tex <==
\subsection{Discussion}
\label{sec:discussion}

In this section, we first discuss the significance and implications of our empirical study's results. We then consider architectural smells from the perspective of technical debt.



==> smell_algorithms.tex <==
\section{Detecting Architectural Smells}
\label{sec:smells_detection}


%Although architectural smells have been discussed in literature, a large-scale empirical study of architectural smells and their impact is still missing. One reason for this is the lack of automated smell detection algorithms: % to find smells. 
%without an efficient way to detect architectural smells from a system's implementation, it is impossible to scale up an empirical study to many systems with many versions. This state of affairs drives us to define detection algorithms for our proposed smell catalog.
%\duc{removed}
This section  describes (1) three smell detection strategies and (2) corresponding detection algorithms for the 11 architectural smells defined in Section \ref{sec:smell_cata}. A detection strategy is a general approach to detect a group of smells. %Smells in each of the four categories are detected based on different detection strategies or combinations of strategies.

%Taking advantage of prior research on specifying and detecting smells at lower abstraction levels (i.e., code and design smells), we made use of the resulting detection strategies. Three popular smell detection approaches \cite{Moha2010.5196681} are lexicon, structure, and measurement. We applied the detection strategies that are related to the characteristics of each smell category. Furthermore, we also selected some of the best-proven practices (e.g., how to select metric thresholds \cite{Lanza:2005:OMP:1076853}) from the literature. 

All architectural-smell detection algorithms have been implemented and %\rhl{integrated into the ARCADE \cite{leempirical}  workbench (recall Section~\ref{sec:related_work}). We have} 
applied 
%\rhl{ARCADE} 
to several systems. %\rhl{, to detect smells in their architectures}. %The selected subject systems are Java-based open-source systems, which allows ARCADE to recover their respective architectures from their source code. Furthermore, %such subject systems are in different software domains to ensure broad applicability of our analysis. E
Each system has a large number of versions, allowing us to study the smells over the evolution of the system. %Furthermore, the selected subject systems have large numbers of reported issues, allowing us to  conduct future studies on how smells impact a system. %We will report the experiment's result in forthcoming studies. 
%\duc{removed}

Specifically, to study the effectiveness, performance, and scalability of our algorithms, we applied them to a total of 421 versions of eight widely used Apache open-source systems: Camel, Continuum, CXF, Hadoop, Nutch, OpenJPA, Struts2, and Wicket. The total amount of code analyzed by our algorithms was 376 MSLOC. Different systems' individual versions ranged in size from 118 KSLOC (Nutch) to 1.96 MSLOC (Hadoop). Average analysis times of our algorithms per system version ranged from few seconds (for \textbf{\uiubsalgname} shown in Algorithm \ref{alg:detectui_ub} below) to 10 minutes (for \textbf{\sdsalgname} shown in Algorithm \ref{alg:detectsd}). %The total number of smells detected for all 1,227 architectural models across the seven systems (i.e., three views---ACDC, ARC, and PKG---per system version)  was 169,667. This averaged to 138 architectural smells per individual system version under a particular architectural view. Our preliminary analysis has also identified that different smells tend to appear with different frequencies, and that those frequencies depend on the system. However, a deeper analysis of such trends and the causes behind them is beyond the scope of this paper; it is part of our on-going work.
For illustration purposes in this section, given the space constraints, we will only highlight one instance of each smell per system. To that end, we selected two Apache systems that contain examples of all 11  smells defined above:  CXF, a widely used open source web services framework, and  Nutch, a large open source web crawler, the parent to  Hadoop.
Table \ref{tab:subject_systems} shows the two subject systems, the respective numbers of versions we analyzed, and the average sizes of each version. %Specifically, we used ARCADE to recover ACDC, ARC, and PKG views of each subject systems' version. The recovered architectures were then used as the input for our detection algorithms to find smell instances. 



% Table generated by Excel2LaTeX from sheet 'Formatted System Stats'
\bgroup
\def\arraystretch{1.25}
\vspace{-5mm}
\begin{table}[h]%[htbp]
	%	\vspace{2.25mm}
	\centering
	\caption{Subject systems analyzed in our study}
		\scriptsize
	%\resizebox{\columnwidth}{!} {
	\begin{tabular}{|p{2cm}|p{2cm}|p{2cm}|p{2cm}|}
		\toprule
		\textbf{System} & \textbf{Domain}   & {\textbf{No. of Versions}} & \textbf{Average SLOC} \\
		\midrule
%		Camel       & Integration Framework  & 78          & 1.13M\\ 
		Apache CXF         & Service Framework      & 120         & 915K \\
%		Hadoop      & Data Process Framework & 63          & 1.96M \\
		Apache Nutch       & Web Crawler      & 21                 & 118K  \\
%		Struts2     & Web App Framework      & 36          & 379K  \\
		%	\midrule
		%	\textbf{Total} &  & \textbf{}    & \textbf{} & \textbf{} \\
		\bottomrule
	\end{tabular}%
	\label{tab:subject_systems}%

\end{table}%

\egroup

%\duc{remove a section}

%\begin{comment}
%\rhl{
\vspace{-10mm}


\vspace{-4mm}
\subsection{Smell Detection Algorithms}

\vspace{-2mm}
\noindent\textbf{Concern-based smells}

\textit{\underline{Scattered Parasitic Functionality (SPF)}}: Algorithm \ref{alg:detectspf}, \spfalgname, %detects \spf by automatically setting a threshold for $\mathit{th_{tc}}$. \spfalgname
returns a map \textit{SPFsmells} where each key in the map is a scattered concern $z$, and each value is a set of at least $\mathit{th_{spf}}$ number of components that have the corresponding key $z$ above the threshold $\mathit{th_{z_c}}$. Lines \ref{alg:detectspf:count_topics:start}-\ref{alg:detectspf:count_topics:end} create a map where keys are concerns and values are the number of components that have that concern above threshold $\mathit{th_{z_c}}$. The $\textit{getConcernsOfComponent}$ function in Line \ref{alg:detectspf:get_concern} returns the topic distribution of the component, which is computed by MALLET. Line \ref{alg:detectspf:th_spf} calculates the threshold $\mathit{th_{z_c}}$ for each component $c$, which helps determine representative topics of a component (Line \ref{alg:detectspf:th_z_c}). Line \ref{alg:detectspf:th_tc} calculates the threshold $\mathit{th_{spf}}$ for the maximum number of concerns in a component. Both thresholds are determined dynamically by the InterQuartile method. Lines \ref{alg:detectspf:detect:start}-\ref{alg:detectspf:detect:end} identify SPF instances by checking if concern \textit{z} appears in at least $th_{spf}$ components (Line \ref{alg:detectspf:th_spf_}).

\label{subsec:detection_algos}
%\vspace{-8mm}
\begin{algorithm}[!th]
	\algsetup{linenosize=\tiny}
	\scriptsize
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
	%	\algsmall
	\caption{\spfalgname}
	\label{alg:detectspf}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	
	
	\KwIn{$C$: a set of components, $T$: a set of system concerns}%, $\mathit{th_{spf}}$: threshold for concern relevance}
	\KwOut{$\mathit{SPFsmells}: $ a map where keys are concerns and values are components}
	
	$\mathit{SPFsmells} \leftarrow$ initialize map as empty\;
	$\mathit{concernCounts} \leftarrow$ initialize all concern counts to 0\;
	\For{$c \in C$}{ \label{alg:detectspf:count_topics:start}
		$T_c \leftarrow \mathit{getConcernsOfComponent(c)}$\; \label{alg:detectspf:get_concern}
		$\mathit{th_{z_c}} \leftarrow \mathit{getHighThreshold(P(T_c))}$\; \label{alg:detectspf:th_spf}
		\For{$z \in T_c$}{
			\If{$P(z \mid c) > \mathit{th_{z_c}}$} { \label{alg:detectspf:th_z_c}
				$\mathit{concernCounts}[z] = \mathit{concernCounts}[z] + 1$\ \label{alg:detectspf:count_topics:end}
			}
		}
	}
	
	%$\mathit{meanConcernCounts} \leftarrow \mathit{computeMean(concernCounts)}$\; \label{alg:detectspf:mean}
	%$\mathit{stdDevOfConcernCounts} \leftarrow \mathit{computeStandardDeviation(concernCounts)}$\;\label{alg:detectspf:stddev}
	%$\mathit{th_{tc}} \leftarrow \mathit{meanConcernCounts} + \mathit{stdDevOfConcernCounts}$
	
	$\mathit{th_{spf}} \leftarrow \mathit{getHighThreshold(concernCounts)}$\; \label{alg:detectspf:th_tc}
	\For{$z \in T$}{ \label{alg:detectspf:detect:start}
		\If{$\mathit{concernCounts[z]} > \mathit{th_{spf}}$} {
			\For{$c \in C$}{
				\If{$P(z \mid c) > \mathit{th_{z_c}}$} { \label{alg:detectspf:th_spf_}
					$\mathit{SPFsmells[z]} \leftarrow \mathit{SPFsmells[z]} \cup \{c\}$\;\label{alg:detectspf:detect:end}
				}
			}
			
		}
	}
	
\end{algorithm}


In most versions of CXF, under the ARC view, we found a Scattered Parasitic Functionality instance where the $org.apache.cxf.BusFactory$ entity and its subclasses are scattered across different components. Even their parent packages are different. Although those classes address the same big concern, which is ``bus'', the subclasses implement different specific concerns. This is the main reason for ARC to assign them to different components. 



%\vspace{-8mm}
\textit{\underline{Concern Overload (CO)}}: Algorithm \ref{alg:detectbco}, \bcoalgname, determines which components in the system have CO. 
The algorithm operates in a manner similar to \spfalgname. \bcoalgname begins by creating a map, $componentConcernCounts$, where keys are components and values are the number of relevant concerns in the component (Lines \ref{alg:detectbco:count_topics:start}-\ref{alg:detectbco:count_topics:end}). While creating the map, threshold $\mathit{th_{z_c}}$ is dynamically computed for each component (Line \ref{alg:detectbco:compute_threshold}) and used to determine prevalent concerns in each component. Later, \bcoalgname uses that map to compute threshold $th_{co}$ in Line  \ref{alg:detectbco:th_t} which is then used to determine which components have the CO smell (Lines \ref{alg:detectbco:detect:start}-\ref{alg:detectbco:detect:end}).

%\vspace{-5mm}	

Like Scattered Parasitic Functionality, we also found a long-lived Concern Overload instance under the ARC view. We found a component that contains the most classes in the $org.apache.cxf.phase$ package. This component implements different steps of information processing in CXF, which include reading a message, transforming it, processing headers and validating the message. Although all these steps are related to message handling, putting all of them into a single component results in the CO smell. 


\begin{algorithm}[!b]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
%	\algsmall
	\scriptsize
	\caption{\bcoalgname}
	\label{alg:detectbco}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of components, $T$: a set of system concerns}%, $\mathit{th_{z_b}}$: threshold for concern relevance}
	\KwOut{$\mathit{COsmells}: $ a set of \bco instances }
	
	$\mathit{COsmells} \leftarrow \emptyset$\;
	$\mathit{componentConcernCounts} \leftarrow$ initialize all brick concern counts to 0\;
	\For{$c \in C$}{ \label{alg:detectbco:count_topics:start}
		$T_c \leftarrow \mathit{getConcernsOfComponent(c)}$\;
		$\mathit{th_{z_c}} \leftarrow \mathit{getHighThreshold(P(T_c))}$\; \label{alg:detectbco:compute_threshold}
		\For{$z \in T_c$}{
			\If{$P(z \mid c) > \mathit{th_{z_c}}$} {
				$\mathit{componentConcernCounts}[c] = \mathit{componentConcernCounts}[c] + 1$\ \label{alg:detectbco:count_topics:end}
			}
		}
	}
	
	%$\mathit{meanBrickConcerns} \leftarrow \mathit{computeMean(brickConcernCounts)}$\; \label{alg:detectbco:mean}
	%$\mathit{stdDevOfBrickConcerns} \leftarrow \mathit{computeStandardDeviation(brickConcernCounts)}$\;\label{alg:detectbco:stddev}
	%$\mathit{th_{t}} \leftarrow \mathit{meanBrickConcerns} + \mathit{stdDevOfBrickConcerns}$
	
	$\mathit{th_{co}} \leftarrow \mathit{getHighThreshold(componentConcernCounts)}$\; \label{alg:detectbco:th_t}
	\For{$c \in C$}{ \label{alg:detectbco:detect:start}
		\If{$\mathit{componentConcernCounts[c]} > \mathit{th_{co}}$} {
			$\mathit{COsmells} \leftarrow \mathit{COsmells} \cup 
			\{c\}$\;\label{alg:detectbco:detect:end}
		}
	}
	
\end{algorithm}

%\vspace{1mm}
\noindent\textbf{Dependency-based smells}
~

\textit{\underline{Dependency Cycle (DC)}}: We detect DC smells by identifying \emph{strongly connected components} in a software system's architectural graph $G = (C,L)$. A strongly connected component is a graph or subgraph where each vertex is reachable from every other vertex. Each strongly connected component in $G$ is a \bdc. Any algorithm that detects strongly connected components \cite{dijkstra1976discipline,leiserson2001introduction} can then be used to identify DC. Therefore, we do not include the detection algorithm for DC in this paper. %\bdcs.

Both Nutch and CXF have one instance of  Dependency  smell starting with their early versions. These instances are persistent throughout both systems' life cycles As both system evolve, the cycles increase in size by involving more components. This observation holds with all three architectural views. 

\begin{comment}
\begin{algorithm}[!th]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
	\algsmall
	\caption{\dcsalgname}
	\label{alg:detectdc}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of components, $L$: links between components}
	\KwOut{$\mathit{DCsmells}: $ a set of \bdc instances }
		
	$\mathit{DCsmells} \leftarrow \emptyset$\;
	$\mathit{L} \leftarrow \emptyset$\;
	$\mathit{componentConcernCounts} \leftarrow$ initialize all brick concern counts to 0\;
	$\mathit{th_{co}} \leftarrow \mathit{detectCycle(G, L)}$\; 
	
\end{algorithm}
\end{comment}



\textit{\underline{Link Overload (LO)}}: Algorithm \ref{alg:detectlo}, \loalgname, extracts the 
LO variants for a set of components $C$ by examining their links $L$. The algorithm 
first determines the number of incoming, outgoing, and combined links per component 
(Lines \ref{alg:detectlo:numlinks:start}-\ref{alg:detectlo:numlinks:end}). 
\loalgname sets the threshold $th_{\mathit{lo}}$ for each variant of LO by computing the thresholds $th_{lo}$ for incoming, outgoing, and combined links (Lines \ref{alg:detectbco:th_lo:start}-\ref{alg:detectbco:th_lo:end})
%\ref{alg:detectlo:stats:start}-\ref{alg:detectlo:stats:end})
. The last part of \loalgname identifies each component and the directionality 
that indicates the variant of LO the component suffers from (Lines 
\ref{alg:detectlo:detect:start}-\ref{alg:detectlo:detect:end}).

\vspace{-7mm}
\begin{algorithm}[!th]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
	%	\algsmall
	\scriptsize
	\caption{\loalgname}
	\label{alg:detectlo}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of components, $L$: links between components}
	\KwOut{$\mathit{LOsmells}: $ a set of \lo instances }
	
	$\mathit{LOsmells} \leftarrow \emptyset$\;
	$\mathit{numLinks} \leftarrow$ initialize map as empty\;
	$\mathit{directionality} \leftarrow \{``in",``out",``both"\}$\;
	
	\For{$c \in C$}{ \label{alg:detectlo:numlinks:start}
		\For{$d \in directionality$} {
			$numLinks[(c,d)] \leftarrow numLinks[(c,d)] + 
			\mathit{getNumLinks(c,d,L)}$\;\label{alg:detectlo:numlinks:end}
		}
	}
	
	\For{$d \in directionality$} { \label{alg:detectbco:th_lo:start}
		%	$\mathit{meanLinks[d]} \leftarrow 
		%	\mathit{computeMean(numLinks,d,B)}$\;\label{alg:detectlo:stats:start}
		%	$\mathit{stdDevLinks[d]} \leftarrow 
		%	\mathit{computeStandardDeviation(numLinks,d,B)}$\;
		%	$\mathit{th_{lo}[d]} \leftarrow \mathit{meanLinks[d]} + 
		%	\mathit{stdDevLinks[d]}$\;\label{alg:detectlo:stats:end}
		$\mathit{th_{lo}[d]} \leftarrow \mathit{getHighThreshold(numLinks,d,C)}$\; \label{alg:detectbco:th_lo:end}
	}
	
	\For{$c \in C$}{ \label{alg:detectlo:detect:start}
		\For{$d \in directionality$} {
			\If{$\mathit{getNumLinks(c,d,L)} > \mathit{th_{lo}[d]}$} {
				$\mathit{LOsmells} \leftarrow \mathit{LOsmells} \cup 
				\{(c,d)\}$\;\label{alg:detectlo:detect:end}
			}
		}
	}
	
\end{algorithm}

\vspace{-8mm}	

In Nutch, we found that some components, especially those which are related to web user interfaces, suffered from Link Overload, such as \seqsplit{$org.apache.nutch.webui.pages.crawls$} or \seqsplit{$org.apache.nutch.webui.pages.instances$} in the PKG view. These components were created with many inner classes within the main classes.


\noindent\textbf{Interface-based smells}

\textit{\underline{Unused Interface (UI)}} and \textit{\underline{Unused Component (UC):}}
As we mentioned in Section \ref{subsec:formal_arch_smells}, UC is the extreme case of UI. Algorithm \ref{alg:detectui_ub}, \textbf{\uiubsalgname}, allows us to detect both of these smells. \textbf{\uiubsalgname} uses the set of links L to determine if an interface has been used or not. The algorithm checks every entity in each component (Lines \ref{alg:detectui_ub:numlinks:start}-\ref{alg:detectui_ub:numlinks:end}), and if an entity has a public interface but no link, then the entity and its parent component are added to the UI instances list. Line \ref{alg:detectui_ub:checkub} uses a boolean flag, \textit{isUB}, to mark that a component does not have UC if at least one entity in the component does not have UI. Line \ref{alg:detectui_ub:addub} checks and adds UC instances to the smell list.

In Nutch, we found that the \textit{SequenceFileInputFormat} class was unused in some 1.x versions (in each view, the parent component of this class was affected by the Unused Interface smell). This class had been removed in version 2.0. We assume that developers noticed and decided to remove this unused class. We could not find any instances of Unused Component in Nutch, but in CXF. Under the PKG view, the $org.apache.cxf.simple$ component had been unused from version 2.0.6 to version 2.2.9. Later, it was used again from version 2.2.10. 


% Unused Interface + Unused Brick
%\vspace{-8mm}
\begin{algorithm}[t]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
%	\algsmall
	\scriptsize
	\caption{\uiubsalgname}
	\label{alg:detectui_ub}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of bricks, $L$: links between components}
	\KwOut{$\mathit{UIsmells}: $ a set of Unused Interface instances, $\mathit{UCsmells}: $ a set of Unused Brick instances }
	
	$\mathit{UIsmells} \leftarrow \emptyset$, 
	$\mathit{UCsmells} \leftarrow \emptyset$\;
	
	\For{$c \in C$}{ \label{alg:detectui_ub:numlinks:start}
		$isUC \leftarrow true$ \\
		\For{$e \in c.E$} {
			\If{$\mathit{getNumInterfaces(e.I)} > 0$} {
				\If{$getNumLinks(e.L)= 0$} {
					$\mathit{UIsmells} \leftarrow \mathit{UIsmells} \cup 
					\{(c,e)\}$\;
				} \label{alg:detectui_ub:numlinks:end}
				\Else{
					$isUC \leftarrow false$ \label{alg:detectui_ub:checkub}
				}
			}
		}
		\If{$isUC$} {
				$\mathit{UCsmells} \leftarrow \mathit{UCsmells} \cup 
			\{(c)\}$\; \label{alg:detectui_ub:addub}
		}
	}
	
\end{algorithm}

\textit{\underline{Sloppy Delegation (SD):}} 

Algorithm \ref{alg:detectsd}, \textbf{\sdsalgname} requires a threshold $th_{sd}$, which defines the minimum number of in-links to consider a delegation appropriate. The algorithm checks every link in each entity (Lines \ref{alg:detectsd:numlinks:start}-\ref{alg:detectsd:numlinks:end}), and if a link has a \textit{`dst'} entity which satisfies the checking condition of SD (defined in Section \ref{subsec:formal_arch_smells}), then the \textit{`dst'} entity and its parent component are added to the list of SD instances (Line \ref{alg:detectsd:addsd}).

In Nutch, we found that $org.apache.nutch.crawl$ and \seqsplit{$org.apache.nutch.scoring.webgraph$} are two components which are heavily affected by the Sloppy Delegation smell. Out of the three architectural views, ACDC provides a better clustering to reduce the number of SD smells. However, those two components still need refactoring. 

% Sloopy Delegation
\vspace{-8mm}
\begin{algorithm}[!bh]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
	%	\algsmall
	\scriptsize
	\caption{\sdsalgname}
	\label{alg:detectsd}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of bricks, $L$: links between components, ~~~~~~~~$\mathit{th_{sd}}$: threshold for relevance delegation}
	\KwOut{$\mathit{smells}: $ a set of Sloppy Delegation instances }
	
	$\mathit{smells} \leftarrow \emptyset$\;
	%	$\mathit{numCouplings} \leftarrow$ initialize map as empty\;
	%	$\mathit{types} \leftarrow \{``fo",``ls"\}$\;
	
	\For{$c_1 \in C$}{ \label{alg:detectsd:numlinks:start}
		\For{$e_1 \in c_1.E$} {
			\For{$l \in e_1.L$}{
				\If{$l.src=e_1$}{\label{alg:detectsd:numlinks:end}
					$e_2 \leftarrow l.dst$\;
					$c_2 \leftarrow getParent(e_2)$\;
					\If{$(e_1 \not\equiv e_2) \land (getOutLink(e_2)=0) $\;
						~~~~~~~~~~~~~~$\land (getInLink(e_2)  <th_{sd})$}{
						$\mathit{smells} \leftarrow \mathit{smells} \cup 
						\{((c_1,e_1),(c_2,e_2))\}$\;
					} \label{alg:detectsd:addsd}
				}
			}
		}
	}
	
\end{algorithm}
\vspace{-7mm}

\textit{\underline{Function Overload (FO)}} and \textit{\underline{Lego Syndrome (LO):}}
These two smells come in a pair, which indicates overloaded and underloaded functionality in components. Algorithm \ref{alg:detectfo_ls}, \textbf{\folsalgname}, allows to us to detect both smells in one run. The algorithm first creates a map between components and their numbers of interfaces (Lines \ref{alg:detectfo_ls:countI:start}-\ref{alg:detectfo_ls:countI:end}). This map then is used to compute two thresholds, $th_{fo}$ and $th_{ls}$, i.e., the high (Line \ref{alg:detectfo_ls:computefo}) and low values (Line \ref{alg:detectfo_ls:computels}) of the inner fences, respectively. Finally, the algorithm revisits each component, checking and adding detected smell instances into two smell lists (Lines \ref{alg:detectfo_ls:check:start}-\ref{alg:detectfo_ls:check:end}). 

Across all 1.x versions of Nutch under the PKG view, we found that one component, \textit{org.apache.nutch.crawl}, has Function Overload and two other components, \textit{org.apache.nutch.net.protocols} and \textit{org.apache.nutch.tool.arc}, have Lego Syndrome.

%Function Overload & Lego Syndrome
\vspace{-2mm}
\begin{algorithm}[!t]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
%	\algsmall
	\scriptsize
	\caption{\folsalgname}
	\label{alg:detectfo_ls}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of bricks, $L$: links between components}
	\KwOut{$\mathit{FOsmells}: $ a set of Functionality Overload , $\mathit{LSsmells}: $a set of Lego Syndrome instances }
	
	$\mathit{FOsmells} \leftarrow \emptyset$, 	$\mathit{LSsmells} \leftarrow \emptyset$\;
	$\mathit{numInterfaces} \leftarrow$ initialize map as empty\;
%	$\mathit{types} \leftarrow \{``fo",``ls"\}$\;
	
	\For{$c \in C$}{ \label{alg:detectfo_ls:countI:start}
		\For{$e \in c.E$} {
		$numInterfaces[c] \leftarrow numInterfaces[c] + 
		\mathit{getNumInterfaces(e.I)}$\;\label{alg:detectdf_cc:numlinks:end}
		}
	} \label{alg:detectfo_ls:countI:end}
	
	$\mathit{th_{fo}} \leftarrow \mathit{getHighThreshold(numInterfaces,C)}$\; \label{alg:detectfo_ls:computefo}
	$\mathit{th_{ls}} \leftarrow \mathit{getLowThreshold(numInterfaces,C)}$\; \label{alg:detectfo_ls:computels}

	
	\For{$c \in C$}{ \label{alg:detectfo_ls:check:start}
		\If{$\mathit{numInterfaces[c]} > \mathit{th_{fo}}$} {
			$\mathit{FOsmells} \leftarrow \mathit{FOsmells} \cup 
			\{(c)\}$\;\label{alg:detectfo_ls:addfo}
		}
		\ElseIf{$\mathit{numInterfaces[c]} < \mathit{th_{ls}}$} {
		$\mathit{LSsmells} \leftarrow \mathit{LSsmells} \cup 
		\{(c)\}$\;\label{alg:detectfo_ls:addls} \label{alg:detectfo_ls:check:end}
	}
	}
	
\end{algorithm}

%\vspace{-7mm}
\begin{algorithm}[!t]
	\renewcommand{\AlCapSty}[1]{\small\small{\textbf{#1}}\unskip}
%	\algsmall
	\scriptsize
	\caption{\dfccalgname}
	\label{alg:detectdf_cc}
	\SetAlgoVlined
	\LinesNumbered 
	\DontPrintSemicolon
	\SetInd{0.3em}{0.6em} 
	
	\KwIn{$C$: a set of bricks, $Cp$: couplings between components}
	\KwOut{$\mathit{DFsmells}: $ a set of Duplicate Functionality , $\mathit{CCsmells}: $a set of Co-change Coupling instances }
	
	$\mathit{DFsmells} \leftarrow \emptyset$, 	$\mathit{CCsmells} \leftarrow \emptyset$, \;
	$\mathit{numDu} \leftarrow$ initialize map as empty\;
	$\mathit{numCo} \leftarrow$ initialize map as empty\;
	
	\For{$c \in C$}{ \label{alg:detectdf_cc:numCouplings:start}
		\For{$e \in e.E$} {
			$numDu[c] \leftarrow numDu[c] + 
			\mathit{getNumDu(c,e.Du)}$\;
			$numCo[c] \leftarrow numCo[c] + 
			\mathit{getNumCo(c,e.Co)}$\;
		} \label{alg:detectdf_cc:numCouplings:end}
	}
	
	$\mathit{th_{df}} \leftarrow \mathit{getHighThreshold(numDu,C)}$\label{alg:detectdf_cc:computedf}\; 
	$\mathit{th_{cc}} \leftarrow \mathit{getHighThreshold(numCo,C)}$\label{alg:detectdf_cc:computecc}\; 
	
	
	\For{$c \in C$}{ \label{alg:detectdf_cc:detect:start}
		\If{$\mathit{numDu[c]} > \mathit{th_{df}}$} {
			$\mathit{DFsmells} \leftarrow \mathit{DFsmells} \cup 
			\{(c)\}$\;
		}
		\If{$\mathit{numCo[c]} > \mathit{th_{cc}}$} {
		$\mathit{CCsmells} \leftarrow \mathit{CCsmells} \cup 
		\{(c)\}$\;
	} \label{alg:detectdf_cc:detect:end}
	}
	
\end{algorithm}

\vspace{2mm}
\noindent\textbf{Coupling-based smells}

\textit{\underline{Duplicate Functionality (DF)}} and \textit{\underline{Co-changes Coupling}} \textit{\underline{(CC):}}
Detecting coupling-based smells is similar to detecting Link Overload. The difference is that the detection algorithms use couplings instead of links as their input. Detecting DF depends on \textit{duplicates}, and detecting CC depends on \textit{co-changes}. Algorithm \ref{alg:detectdf_cc}, \dfccalgname, shows how to detect these two types of smells. The algorithm first creates two maps between components and their numbers of duplicates as well as co-changes (Lines \ref{alg:detectdf_cc:numCouplings:start}-\ref{alg:detectdf_cc:numCouplings:end}). \dfccalgname uses these maps to compute two thresholds, $th_{df}$ and $th_{cc}$, which are the high inner-fence values (Lines \ref{alg:detectdf_cc:computedf}-\ref{alg:detectdf_cc:computecc}). Finally, the algorithm visits each component again, checks and adds detected smell instances into two smell lists (Lines \ref{alg:detectdf_cc:detect:start}-\ref{alg:detectdf_cc:detect:end}).

Under the PKG view of CXF, we found that the component \textit{org.apache.cxf.interceptor} has the Co-changes Coupling smell along with 6 other components in version 2.x. Later on, one CC instance has been removed in version 3.x. However, new CC smell instances were also introduced. We also found \seqsplit{$org.apache.cxf.ws.security.wss4j.policyvalidators$} and $org.apache.cxf.jibx$ to be strongly affected by Duplicate Functionality. Almost all entities in those two components have duplications with entities in other components.



%Although the smells' definitions are agnostic to the programming language used to implement a system, details of smell detection algorithms are slightly different and depend on the language. In this paper, the implementation of smell detection algorithms based on the assumption that the software is written
%The eleven smells defined in the previous section are representative of both (1) architectural smells in general and (2) the manner in which architectural-smell definitions can be transformed to detection algorithms. 
%Our formalization of architectural concepts and architectural-smell definitions in Section \ref{sec:smell_cata} allows us to build algorithms for detecting each of the architectural smells. The limited number of components, links, and concerns afforded by employing an architectural level of abstraction allows our detection algorithms to be simple and efficient. 


==> smell_formalization.tex <==
%\vspace{-3mm}
\section{Selecting, Capturing, and Detecting  Smells}
\label{sec:smell_cata}





